Optically Resolved Excited State Hyperfine Structure of a Silicon Colour Centre in the Telecom Bands

Nuclear spin qubits in silicon offer exceptionally coherent quantum memory, and optically-interfaced spins are a promising platform for both quantum networking and distributed quantum computing. It has been proposed that emitters with diamagnetic ground states may permit an optical interface to nuclear spin memories via metastable, hyperfine-coupled excited states while suppressing key sources of decoherence. Until now, direct optical observation of suitable transitions in silicon colour centres has remained elusive. Here we characterize the singly-ionized interstitial aluminum donor (Al$_\mathrm{i}^+$) in isotopically purified $^{28}$Si and find several novel features of this little-studied defect. We measure bright emission and strong optical transitions and, in contrast to previous studies of this centre, attribute its emission to an exchange-split spin triplet and singlet level of the lowest-energy 1s:T$_2$ excited state. We measure the excited-state lifetimes and, as a consequence of its narrow emission linewidth, observe the fine and hyperfine structure of the long-lived triplet state. This constitutes the first measurement of an optically-resolved hyperfine structure in the excited state of a telecommunications-band silicon colour centre.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}



